Virgo Detector Characterization and Data Quality: tools

Detector characterization and data quality studies -- collectively referred to as {\em DetChar} activities in this article -- are paramount to the scientific exploitation of the joint dataset collected by the LIGO-Virgo-KAGRA global network of ground-based gravitational-wave (GW) detectors. They take place during each phase of the operation of the instruments (upgrade, tuning and optimization, data taking), are required at all steps of the dataflow (from data acquisition to the final list of GW events) and operate at various latencies (from near real-time to vet the public alerts to offline analyses). This work requires a wide set of tools which have been developed over the years to fulfill the requirements of the various DetChar studies: data access and bookkeeping; global monitoring of the instruments and of the different steps of the data processing; studies of the global properties of the noise at the detector outputs; identification and follow-up of noise peculiar features (whether they be transient or continuously present in the data); quick processing of the public alerts. The present article reviews all the tools used by the Virgo DetChar group during the third LIGO-Virgo Observation Run (O3, from April 2019 to March 2020), mainly to analyse the Virgo data acquired at EGO. Concurrently, a companion article focuses on the results achieved by the DetChar group during the O3 run using these tools.

==> definitions.tex <==
\usepackage{graphicx}
\usepackage{color}
\usepackage{xcolor}
\usepackage{epsfig}
\usepackage{float}
\usepackage{multirow}
\expandafter\let\csname equation*\endcsname\relax
\expandafter\let\csname endequation*\endcsname\relax
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{tabularx,url,color}
\usepackage[colorlinks=true]{hyperref}
\usepackage[T1]{fontenc}

\usepackage{lineno}
\usepackage{upgreek}

\usepackage{tocloft}

\usepackage{acro}

\usepackage{longtable}

\RequirePackage{xspace}

\newcommand\rednote[1]{\textcolor{red}{\bf {#1}}}
\newcommand\bluenote[1]{\textcolor{blue}{\bf {#1}}}

\newcommand{\Reviewer}[1]{~\\ \noindent {\textcolor{purple}{\bf {Reviewer(s): #1}}} \\}
\newcommand{\Writer}[1]{~\\ \noindent {\textcolor{blue}{\bf {Writer(s): #1}}} \\}

\newenvironment{oldtext}{~\\ \color{olive}{\bf $<$OLDTEXT$>$}}{\bf $<$/OLDTEXT$>$ ~\\}

\usepackage[normalem]{ulem}
\usepackage{soul}

\usepackage{orcidlink}

\makeatletter
\newcommand{\mainmatter}{%
  \setcounter{footnote}{0}%
  \patchcmd{\@makefntext}{\fnsymbol}{\arabic}{}{}%
  \patchcmd{\@thefnmark}{\fnsymbol}{\arabic}{}{}%
  \def\@makefnmark{\textsuperscript{\arabic{footnote}}}%
}
\makeatother

\endinput

